Understanding and Supporting Debugging Workflows in Multiverse Analysis

Multiverse analysis, a paradigm for statistical analysis that considers all combinations of reasonable analysis choices in parallel, promises to improve transparency and reproducibility. Although recent tools help analysts specify multiverse analyses, they remain difficult to use in practice. In this work, we identify debugging as a key barrier due to the latency from running analyses to detecting bugs and the scale of metadata processing needed to diagnose a bug. To address these challenges, we prototype a command-line interface tool, Multiverse Debugger, which helps diagnose bugs in the multiverse and propagate fixes. In a qualitative lab study (n=13), we use Multiverse Debugger as a probe to develop a model of debugging workflows and identify specific challenges, including difficulty in understanding the multiverse's composition. We conclude with design implications for future multiverse analysis authoring systems.

==> 0-figures-and-tables.tex <==

\newcommand{\tableDefinitions}{
\begin{table}
  \caption{Relevant Multiverse Analysis Definitions}
  \label{tab:definitions}
  \begin{tabular}{cl}
    \toprule
    Term & Definition\\
    \midrule
     Decision & \makecell{Any decision that is reasonable and defensible an analyst may consider in an analysis. \\ &(e.g., Statistical Model, Data Filtering etc.)} \\
     Decision Option & The alternatives an analyst considers in a decision. (e.g., bayesian model, frequentist model etc.) \\
     Universe & A single end-to-end analysis representing one combination of decision options \\
     Multiverse & A collection of all universes as specified by a set of decisions and their decision options\\
  \bottomrule
\end{tabular}
\end{table}
}


==> 4-formative.tex <==
\section{Formative Study}
\label{formative}

In this section, we describe our formative user study, which offers insight into the perspectives of multiverse practitioners and multiverse tool developers on key challenges of multiverse analysis. Based on their perspectives, we identify multiverse debugging as a fundamental challenge that currently is not well supported by existing tools, and we develop an initial model of multiverse debugging workflows and associated challenges.
This initial model informs our design motivations and a prototype tool to help explore multiverse debugging workflows and how to best support them (\autoref{sec:tool}). 
Accordingly, we conduct a study specifically focused on multiverse debugging (\autoref{sec:focused_study}), discuss results (\autoref{sec:label_results}) and describe key design implications (\autoref{sec:discussion}). 



\subsection{Interviews with Two Multiverse Practitioners}
\label{subsec:formative_study_practitioners}
Prior work \cite{liu_boba_2021, dragicevic_increasing_2019, liu_paths_2020} and our own experiences informed our early understanding that multiverse authoring is generally difficult. 
To identify specific challenges in authoring and conducting multiverse analyses, we first conduct in-depth interview studies with two researchers who have recently authored multiverse analyses. We found these researchers through our collaboration networks. Neither relied on existing multiverse tools. Instead,
they wrote custom scripts that generated each universe script. During the interviews, which lasted for
approximately two hours each, the researchers walked us through their analyses,
including their scripts, findings, and any historical artifacts from their git repository 
histories. 
Without being prompted, 
both brought up how challenging finding and propagating bug fixes is for them.

We learned that the researchers approach authoring multiverse analyses in a
bottom-up, iterative fashion. They focus on a few key decisions and
options, consult their peers and supervisors, and then add additional
decisions and options based on their team's input. This iterative nature
requires keeping track of which combinations of decision options were
previously considered and how, if at all, the results have altered since
changing or adding decisions and decision options. The same process applies when the
researchers encounter and fix bugs. They must identify bugs, fix decision
options that introduce the bugs, and then re-run their multiverse analyses
to see how the bugs impact their results. 

The core activities involved in
finding and fixing bugs are to: 
(i) identify decision options that are causing error messages or
unexpected results, which often involve focusing on a single combination of
decision options (a universe) at a time and (ii) abstract code fixes in a universe and 
propagate to other relevant universes, which involves updating their
universe-generating scripts. This led to an understanding that multiverse debugging is a key challenge and that resolving difficulties surrounding this process could make it easier to author multiverse analyses more generally.



\subsection{Additional Correspondences with Experienced Multiverse Tool Developers}
We cross-examined our observed challenges and insights in debugging with two independent, experienced
researchers who have authored multiverse analyses and developed multiverse
analysis tools.  We corresponded with
these researchers via email. 

Both researchers corroborated the importance of
starting with a single universe and then propagating changes to the rest of the
universes: \shortquote{I may
look at a single universe. Then I apply the solution to all affected paths.
Currently, this can only be achieved by modifying the multiverse
specification.} The other researcher had a similar debugging process: \shortquote{I
always debug by looking at individual universe scripts that instantiate a
particular set of decisions that I think might be involved in the error}.
They also mentioned how debugging multiverse analyses is like debugging a
single universe but with \shortquote{the added difficulty of figuring out why
the bugs come up in a particular analysis}. Finally, one tool developer also highlighted the additional steps needed to pinpoint an error: \shortquote{I often read the error messages and pick a specific error to focus on. Then I examine all paths that lead to a specific error to distill commonality.} 


\initWorkflowFig

\subsection{Workflow Model Informed by Formative Work}
\label{subsec:workflow_model_exploratory}
 The findings from our formative study reveal debugging as a central challenge to multiverse analysis authoring, which is consistent with prior work on multiverse authoring that identified current tools have not yet addressed debugging challenges~\cite{sarma_multiverse_2021}. 
 Guided by these findings and our own experiences using existing tools, we hypothesize a common multiverse debugging workflow (\autoref{fig:debug_workflow}). The workflow model is an initial attempt to understand debugging in multiverse analysis and contrasts with the multiverse authoring workflow that is currently supported through existing tools (\autoref{fig:debug_workflow}A). After specifying and compiling a multiverse specification, the analyst executes the universes which produces error messages (\autoref{fig:debug_workflow}D1). Next, the analyst tries to diagnose the cause of the bug, which leads them to a single buggy universe to target (\autoref{fig:debug_workflow}D2). This step often involves examining multiple universes that share an error message. Once the analyst is working with an individual universe, they address the bug and make edits along the way, the same as they would when debugging a single script (\autoref{fig:debug_workflow}D3). After, they abstract and propagate the specific changes in the universe back to the higher-level multiverse specification (\autoref{fig:debug_workflow}D4). Finally, after the edits are propagated to form a new multiverse specification, it is compiled (\autoref{fig:debug_workflow}D5). This iterative debugging cycle typically repeats multiple times until all bugs are addressed.
 
 From our initial workflow model, we identify three additional challenges beyond debugging a single analysis.
 
 \xhdr{Challenge 1 - Detecting bugs is slow} During execution of the multiverse (\autoref{fig:debug_workflow}D1), the order of execution of the universes is arbitrary. Therefore, to discover a bug that occurs in a select few universes, hundreds or thousands of universes may need to be executed before the buggy universe is encountered. Even with running universes in parallel, this process can be time consuming and drastically slows down the debugging cycle.
 
 \xhdr{Challenge 2 - Sifting through error messages and multiverse artifacts to diagnose a bug is difficult at scale} In the process of diagnosing an error from running the multiverse (\autoref{fig:debug_workflow}D2), an analyst potentially needs to navigate through many error messages, many universes, and the specification summary and relate these sources to understand the shared decision options of an error. It is infeasible for an analyst to inspect hundreds of files (or a single file that combines these) and looking at a significantly smaller subset may not fully isolate the shared decision options of an error and divert focus from the true source of a bug. We note that a multiverse that does not lead to any error messages is not necessarily bug free. For example, a poorly specified model formula may not be statistically sound but may not raise any error messages. However, many bugs exhibit themselves as error messages and that is the primary way the researchers in our formative study used to debug.

 
 \xhdr{Challenge 3 - Abstracting and propagating universe edits to the multiverse increases cognitive load} In the procedure to abstract and propagate universe edits to the multiverse specification (\autoref{fig:debug_workflow}D4), the analyst needs to remember all their edits and locate where to place them in the multiverse specification. In complex multiverse specifications and universe edits that involve many changes, propagating universe edits induces additional cognitive demands, especially when the analyst must keep track of the associated decision options underlying the code they are propagating. 



==> main-design-motivation.tex <==
\section{Design Motivation}
\label{sec:designMotivation}
Based on the formative study study in \autoref{formative}, we identify three design goals to support analysts in the multiverse debugging workflow (\autoref{fig:debug_workflow}). The goals correspond to addressing the three challenges identified in \autoref{subsec:workflow_model_exploratory}. 

\begin{enumerate}
    \item \textit{DG 1 - Reduce the time between executing universes and encountering errors.}
    After compiling a multiverse specification, a tool should enable analysts to quickly observe errors before committing to running the full multiverse. This is in the spirit of unit testing in which different components of the multiverse is rapidly tested before running the entire system. Quickly identifying errors before executing an entire multiverse may reduce time spent authoring (buggy) multiverse analyses.
    
    \item \textit{DG 2 - Give an overview of errors and how they relate to specific
    decision options.} Running thousands of universes can lead to thousands of individual error logs. In addition, errors may arise due to a combination of decision options, which the analyst did not test when writing the multiverse specification. Therefore, diagnosing the severity and frequency of an error helps to identify which parts of the code may need to be updated (including adding or removing dependencies between decision options in the multiverse specification). 
    % \tim{review previous sentence for accuracy}
    % is necessary to update code, which may impose or remove new dependencies between decision options. 
    To identify common bugs and distinguish among
    different kinds of bugs, summarizing the frequency of errors and connecting
    them to specific decisions and decision options are likely to help
    analysts.
    \item \textit{DG 3 - Support the abstraction and propagation of single universe error fixes to a multiverse specification} The context of a
    multiverse analysis adds new complexity to fixing errors. Analysts may elect to debug errors in a specific universe as opposed to the higher-level multiverse specification. This enables analysts to take advantage of already familiar and idiosyncratic ways of debugging specific universe errors. In the analysts process of debugging a single universe, they can leverage an entire ecosystem of single script debugging tools that they may already be familiar with. Therefore, making the process of propagating changes to individual universes to the higher-level multiverse specification easier, empowers the single universe debugging workflow. 
    
\end{enumerate}
